Evaporating sessile droplets: solutal Marangoni effects overwhelm thermal Marangoni flow

When an evaporating water droplet is deposited on a thermally conductive substrate, the minimum temperature will be at the apex due to evaporative cooling. Consequently, density and surface tension gradients emerge within the droplet and at the droplet-gas interface, giving rise to competing flows from, respectively, the apex towards the contact line (thermal-buoyancy-driven flow) and the other way around (thermal Marangoni flow). In small droplets with a diameter below the capillary length, the thermal Marangoni effects are expected to dominate over thermal buoyancy ("thermal Rayleigh") effects. However, contrary to these theoretical predictions, our experiments mostly show a dominant circulation from the apex towards the contact line, indicating a prevailing of thermal Rayleigh convection. Furthermore, our experiments often show an unexpected asymmetric flow that persisted for several minutes. We hypothesise that a tiny amount of contaminants, commonly encountered in experiments with water/air interfaces, act as surfactants and counteract the thermal surface tension gradients at the interface and thereby promote the dominance of Rayleigh convection. Our finite element numerical simulations demonstrate that, under our specified experimental conditions, a mere 0.5% reduction in the static surface tension caused by surfactants leads to a reversal in the flow direction, compared to the theoretical prediction without contaminants. Additionally, we investigate the linear stability of the axisymmetric solutions, revealing that the presence of surfactants also affects the axial symmetry of the flow.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
